Emulating a large memory with a collection of small ones

Sequential computation is well understood but does not scale well with current technology. Within the next decade, systems will contain large numbers of processors with potentially thousands of processors per chip. Despite this, many computational problems exhibit little or no parallelism and many existing formulations are sequential. It is therefore essential that highly-parallel architectures can support sequential computation by emulating large memories with collections of smaller ones, thus supporting efficient execution of sequential programs or sequential components of parallel programs. This paper demonstrates that a realistic parallel architecture with scalable low-latency communications can execute large-memory sequential programs with a factor of only 2 to 3 slowdown, when compared to a conventional sequential architecture. This overhead seems an acceptable price to pay to be able to switch between executing highly-parallel programs and sequential programs with large memory requirements. Efficient emulation of large memories could therefore facilitate a transition from sequential machines by allowing existing programs to be compiled directly to a highly-parallel architecture and then for their performance to be improved by exploiting parallelism in memory accesses and computation.

==> Makefile <==
pdflatex=pdflatex -interaction=errorstopmode -halt-on-error -shell-escape

files=\
	preamble.tex \
	emulation.tex \
	introduction.tex \
	implementation.tex \
	results.tex \
	refs.bib

all: full

full: $(files)
	$(pdflatex) emulation
	make -f emulation.makefile
	bibtex emulation
	$(pdflatex) emulation
	$(pdflatex) emulation

once: $(files)
	$(pdflatex) emulation

clean:
	rm -f emulation.pdf
	rm -f *.aux *.log *.toc *.blg *.bbl *.figlist *.makefile *.out *.pdf
	rm -f model/*.dat
	rm -f model/*.pyc
	rm -f results/model/*.dat
	rm -f figures/cache/*


==> results/emulation/access-latency-4096-rand-nordma.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,1341){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(726,1525){\makebox(0,0)[r]{\strut{} 20}}%
      \csname LTb\endcsname%
      \put(726,1709){\makebox(0,0)[r]{\strut{} 40}}%
      \csname LTb\endcsname%
      \put(726,1892){\makebox(0,0)[r]{\strut{} 60}}%
      \csname LTb\endcsname%
      \put(726,2076){\makebox(0,0)[r]{\strut{} 80}}%
      \csname LTb\endcsname%
      \put(726,2260){\makebox(0,0)[r]{\strut{} 100}}%
      \csname LTb\endcsname%
      \put(726,2444){\makebox(0,0)[r]{\strut{} 120}}%
      \csname LTb\endcsname%
      \put(726,2628){\makebox(0,0)[r]{\strut{} 140}}%
      \csname LTb\endcsname%
      \put(726,2811){\makebox(0,0)[r]{\strut{} 160}}%
      \csname LTb\endcsname%
      \put(726,2995){\makebox(0,0)[r]{\strut{} 180}}%
      \csname LTb\endcsname%
      \put(726,3179){\makebox(0,0)[r]{\strut{} 200}}%
      \csname LTb\endcsname%
      \put(858,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}8}}}%
      \csname LTb\endcsname%
      \put(1147,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}16}}}%
      \csname LTb\endcsname%
      \put(1437,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}32}}}%
      \csname LTb\endcsname%
      \put(1726,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}64}}}%
      \csname LTb\endcsname%
      \put(2016,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}128}}}%
      \csname LTb\endcsname%
      \put(2305,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}256}}}%
      \csname LTb\endcsname%
      \put(2595,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}512}}}%
      \csname LTb\endcsname%
      \put(2884,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}1024}}}%
      \csname LTb\endcsname%
      \put(3174,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}2048}}}%
      \csname LTb\endcsname%
      \put(3463,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}4096}}}%
      \put(220,2260){\rotatebox{-270}{\makebox(0,0){\strut{}Overhead (ns)}}}%
      \put(2160,814){\makebox(0,0){\strut{}Size of emulation (tiles)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1670,393){\makebox(0,0)[r]{\strut{}Clos 1K tiles}}%
      \csname LTb\endcsname%
      \put(1670,173){\makebox(0,0)[r]{\strut{}Mesh 1K tiles}}%
      \csname LTb\endcsname%
      \put(3018,393){\makebox(0,0)[r]{\strut{}Clos 4K tiles}}%
      \csname LTb\endcsname%
      \put(3018,173){\makebox(0,0)[r]{\strut{}Mesh 4K tiles}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{results/emulation/access-latency-4096-rand-nordma_img.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/emulation/access-latency-4096-rand.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(726,1341){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(726,1647){\makebox(0,0)[r]{\strut{} 100}}%
      \csname LTb\endcsname%
      \put(726,1954){\makebox(0,0)[r]{\strut{} 200}}%
      \csname LTb\endcsname%
      \put(726,2260){\makebox(0,0)[r]{\strut{} 300}}%
      \csname LTb\endcsname%
      \put(726,2566){\makebox(0,0)[r]{\strut{} 400}}%
      \csname LTb\endcsname%
      \put(726,2873){\makebox(0,0)[r]{\strut{} 500}}%
      \csname LTb\endcsname%
      \put(726,3179){\makebox(0,0)[r]{\strut{} 600}}%
      \csname LTb\endcsname%
      \put(858,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}8}}}%
      \csname LTb\endcsname%
      \put(1147,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}16}}}%
      \csname LTb\endcsname%
      \put(1437,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}32}}}%
      \csname LTb\endcsname%
      \put(1726,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}64}}}%
      \csname LTb\endcsname%
      \put(2016,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}128}}}%
      \csname LTb\endcsname%
      \put(2305,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}256}}}%
      \csname LTb\endcsname%
      \put(2595,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}512}}}%
      \csname LTb\endcsname%
      \put(2884,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}1024}}}%
      \csname LTb\endcsname%
      \put(3174,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}2048}}}%
      \csname LTb\endcsname%
      \put(3463,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}4096}}}%
      \put(220,2260){\rotatebox{-270}{\makebox(0,0){\strut{}Access latency (ns)}}}%
      \put(2160,814){\makebox(0,0){\strut{}Size of emulation (tiles)}}%
      \put(3502,1451){\makebox(0,0)[l]{\strut{}DDR3}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1670,393){\makebox(0,0)[r]{\strut{}Clos 1K tiles}}%
      \csname LTb\endcsname%
      \put(1670,173){\makebox(0,0)[r]{\strut{}Mesh 1K tiles}}%
      \csname LTb\endcsname%
      \put(3018,393){\makebox(0,0)[r]{\strut{}Clos 4K tiles}}%
      \csname LTb\endcsname%
      \put(3018,173){\makebox(0,0)[r]{\strut{}Mesh 4K tiles}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{results/emulation/access-latency-4096-rand_img.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/emulation/access-latency-4096-sp-nordma.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(594,1341){\makebox(0,0)[r]{\strut{} 0}}%
      \csname LTb\endcsname%
      \put(594,1604){\makebox(0,0)[r]{\strut{} 10}}%
      \csname LTb\endcsname%
      \put(594,1866){\makebox(0,0)[r]{\strut{} 20}}%
      \csname LTb\endcsname%
      \put(594,2129){\makebox(0,0)[r]{\strut{} 30}}%
      \csname LTb\endcsname%
      \put(594,2391){\makebox(0,0)[r]{\strut{} 40}}%
      \csname LTb\endcsname%
      \put(594,2654){\makebox(0,0)[r]{\strut{} 50}}%
      \csname LTb\endcsname%
      \put(594,2916){\makebox(0,0)[r]{\strut{} 60}}%
      \csname LTb\endcsname%
      \put(594,3179){\makebox(0,0)[r]{\strut{} 70}}%
      \csname LTb\endcsname%
      \put(726,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}8}}}%
      \csname LTb\endcsname%
      \put(1030,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}16}}}%
      \csname LTb\endcsname%
      \put(1334,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}32}}}%
      \csname LTb\endcsname%
      \put(1638,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}64}}}%
      \csname LTb\endcsname%
      \put(1942,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}128}}}%
      \csname LTb\endcsname%
      \put(2247,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}256}}}%
      \csname LTb\endcsname%
      \put(2551,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}512}}}%
      \csname LTb\endcsname%
      \put(2855,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}1024}}}%
      \csname LTb\endcsname%
      \put(3159,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}2048}}}%
      \csname LTb\endcsname%
      \put(3463,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}4096}}}%
      \put(220,2260){\rotatebox{-270}{\makebox(0,0){\strut{}Overhead (ns)}}}%
      \put(2094,814){\makebox(0,0){\strut{}Size of emulation (tiles)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1604,393){\makebox(0,0)[r]{\strut{}Clos 1K tiles}}%
      \csname LTb\endcsname%
      \put(1604,173){\makebox(0,0)[r]{\strut{}Mesh 1K tiles}}%
      \csname LTb\endcsname%
      \put(2952,393){\makebox(0,0)[r]{\strut{}Clos 4K tiles}}%
      \csname LTb\endcsname%
      \put(2952,173){\makebox(0,0)[r]{\strut{}Mesh 4K tiles}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{results/emulation/access-latency-4096-sp-nordma_img.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/emulation/synthetic-dhrystone-rand.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(594,1341){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%
      \put(594,1604){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%
      \put(594,1866){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%
      \put(594,2129){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%
      \put(594,2391){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%
      \put(594,2654){\makebox(0,0)[r]{\strut{}6.0}}%
      \csname LTb\endcsname%
      \put(594,2916){\makebox(0,0)[r]{\strut{}7.0}}%
      \csname LTb\endcsname%
      \put(594,3179){\makebox(0,0)[r]{\strut{}8.0}}%
      \csname LTb\endcsname%
      \put(726,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}8}}}%
      \csname LTb\endcsname%
      \put(1030,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}16}}}%
      \csname LTb\endcsname%
      \put(1334,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}32}}}%
      \csname LTb\endcsname%
      \put(1638,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}64}}}%
      \csname LTb\endcsname%
      \put(1942,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}128}}}%
      \csname LTb\endcsname%
      \put(2247,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}256}}}%
      \csname LTb\endcsname%
      \put(2551,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}512}}}%
      \csname LTb\endcsname%
      \put(2855,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}1024}}}%
      \csname LTb\endcsname%
      \put(3159,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}2048}}}%
      \csname LTb\endcsname%
      \put(3463,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}4096}}}%
      \put(220,2260){\rotatebox{-270}{\makebox(0,0){\strut{}Slowdown}}}%
      \put(2094,814){\makebox(0,0){\strut{}Size of emulation (tiles)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1604,393){\makebox(0,0)[r]{\strut{}Clos 1K tiles}}%
      \csname LTb\endcsname%
      \put(1604,173){\makebox(0,0)[r]{\strut{}Mesh 1K tiles}}%
      \csname LTb\endcsname%
      \put(2952,393){\makebox(0,0)[r]{\strut{}Clos 4K tiles}}%
      \csname LTb\endcsname%
      \put(2952,173){\makebox(0,0)[r]{\strut{}Mesh 4K tiles}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{results/emulation/synthetic-dhrystone-rand_img.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/emulation/synthetic-range-clos-rand.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(594,1121){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%
      \put(594,1464){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%
      \put(594,1807){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%
      \put(594,2150){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%
      \put(594,2493){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%
      \put(594,2836){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%
      \put(594,3179){\makebox(0,0)[r]{\strut{}6.0}}%
      \csname LTb\endcsname%
      \put(726,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}8}}}%
      \csname LTb\endcsname%
      \put(1030,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}16}}}%
      \csname LTb\endcsname%
      \put(1334,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}32}}}%
      \csname LTb\endcsname%
      \put(1638,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}64}}}%
      \csname LTb\endcsname%
      \put(1942,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}128}}}%
      \csname LTb\endcsname%
      \put(2247,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}256}}}%
      \csname LTb\endcsname%
      \put(2551,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}512}}}%
      \csname LTb\endcsname%
      \put(2855,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}1024}}}%
      \csname LTb\endcsname%
      \put(3159,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}2048}}}%
      \csname LTb\endcsname%
      \put(3463,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}4096}}}%
      \put(220,2150){\rotatebox{-270}{\makebox(0,0){\strut{}Slowdown}}}%
      \put(2094,594){\makebox(0,0){\strut{}Size of emulation (tiles)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(956,173){\makebox(0,0)[r]{\strut{}0\%}}%
      \csname LTb\endcsname%
      \put(1604,173){\makebox(0,0)[r]{\strut{}5\%}}%
      \csname LTb\endcsname%
      \put(2252,173){\makebox(0,0)[r]{\strut{}15\%}}%
      \csname LTb\endcsname%
      \put(2900,173){\makebox(0,0)[r]{\strut{}50\%}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{results/emulation/synthetic-range-clos-rand_img.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/emulation/synthetic-range-mesh-rand.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(594,1121){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%
      \put(594,1464){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%
      \put(594,1807){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%
      \put(594,2150){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%
      \put(594,2493){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%
      \put(594,2836){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%
      \put(594,3179){\makebox(0,0)[r]{\strut{}6.0}}%
      \csname LTb\endcsname%
      \put(726,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}8}}}%
      \csname LTb\endcsname%
      \put(1030,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}16}}}%
      \csname LTb\endcsname%
      \put(1334,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}32}}}%
      \csname LTb\endcsname%
      \put(1638,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}64}}}%
      \csname LTb\endcsname%
      \put(1942,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}128}}}%
      \csname LTb\endcsname%
      \put(2247,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}256}}}%
      \csname LTb\endcsname%
      \put(2551,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}512}}}%
      \csname LTb\endcsname%
      \put(2855,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}1024}}}%
      \csname LTb\endcsname%
      \put(3159,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}2048}}}%
      \csname LTb\endcsname%
      \put(3463,989){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}4096}}}%
      \put(220,2150){\rotatebox{-270}{\makebox(0,0){\strut{}Slowdown}}}%
      \put(2094,594){\makebox(0,0){\strut{}Size of emulation (tiles)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(956,173){\makebox(0,0)[r]{\strut{}0\%}}%
      \csname LTb\endcsname%
      \put(1604,173){\makebox(0,0)[r]{\strut{}5\%}}%
      \csname LTb\endcsname%
      \put(2252,173){\makebox(0,0)[r]{\strut{}15\%}}%
      \csname LTb\endcsname%
      \put(2900,173){\makebox(0,0)[r]{\strut{}50\%}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{results/emulation/synthetic-range-mesh-rand_img.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/emulation/xcmp-time-rand.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3968.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(594,1341){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%
      \put(594,1545){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%
      \put(594,1749){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%
      \put(594,1954){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%
      \put(594,2158){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%
      \put(594,2362){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%
      \put(594,2566){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%
      \put(594,2771){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%
      \put(594,2975){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%
      \put(594,3179){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%
      \put(726,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}8}}}%
      \csname LTb\endcsname%
      \put(1030,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}16}}}%
      \csname LTb\endcsname%
      \put(1334,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}32}}}%
      \csname LTb\endcsname%
      \put(1638,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}64}}}%
      \csname LTb\endcsname%
      \put(1942,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}128}}}%
      \csname LTb\endcsname%
      \put(2247,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}256}}}%
      \csname LTb\endcsname%
      \put(2551,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}512}}}%
      \csname LTb\endcsname%
      \put(2855,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}1024}}}%
      \csname LTb\endcsname%
      \put(3159,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}2048}}}%
      \csname LTb\endcsname%
      \put(3463,1209){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}4096}}}%
      \put(220,2260){\rotatebox{-270}{\makebox(0,0){\strut{}Slowdown}}}%
      \put(2094,814){\makebox(0,0){\strut{}Size of emulation (tiles)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1604,393){\makebox(0,0)[r]{\strut{}Clos 1K tiles}}%
      \csname LTb\endcsname%
      \put(1604,173){\makebox(0,0)[r]{\strut{}Mesh 1Ki tiles}}%
      \csname LTb\endcsname%
      \put(3084,393){\makebox(0,0)[r]{\strut{}Clos 4K tiles}}%
      \csname LTb\endcsname%
      \put(3084,173){\makebox(0,0)[r]{\strut{}Mesh 4Ki tiles}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{results/emulation/xcmp-time-rand_img.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup

